Use of Graph Neural Networks in Aiding Defensive Cyber Operations

In an increasingly interconnected world, where information is the lifeblood of modern society, regular cyber-attacks sabotage the confidentiality, integrity, and availability of digital systems and information. Additionally, cyber-attacks differ depending on the objective and evolve rapidly to disguise defensive systems. However, a typical cyber-attack demonstrates a series of stages from attack initiation to final resolution, called an attack life cycle. These diverse characteristics and the relentless evolution of cyber attacks have led cyber defense to adopt modern approaches like Machine Learning to bolster defensive measures and break the attack life cycle. Among the adopted ML approaches, Graph Neural Networks have emerged as a promising approach for enhancing the effectiveness of defensive measures due to their ability to process and learn from heterogeneous cyber threat data. In this paper, we look into the application of GNNs in aiding to break each stage of one of the most renowned attack life cycles, the Lockheed Martin Cyber Kill Chain. We address each phase of CKC and discuss how GNNs contribute to preparing and preventing an attack from a defensive standpoint. Furthermore, We also discuss open research areas and further improvement scopes.

==> commented-text.tex <==
% Graph convolutional networks (GCNs) are mimics CNNs, modern GCNs learn the common local and global structural patterns of graphs through designed convolution and readout functions. Because most GCNs can be trained with task-specific loss via backpropagation. We first discuss the convolution operations, then move to the readout operations and some other improvements. Using graph convolution operations, useful node features can be learned to solve many node-focused tasks. However, to tackle graph-focused tasks, node information needs to be aggregated to form a graph-level representation. In the literature, such procedures are usually called the readout operations. Based on a regular and local neighborhood, standard CNNs conduct multiple stride convolutions or poolings to gradually reduce the resolution. Since graphs lack a grid structure, these existing methods cannot be used directly.

% In this section, we revisit a variant of artificial neural network that is formed by a feed-forward neural network but has recurrent units. These recurrent units helps to retain historical states that helps in future predictions. Recurrent neural network (RNN) is commonly used to learn temporal or data that involves time sequences. RNNs are distinguished by their memory to retain history as they take information from prior inputs to influence the current input and output. While traditional deep neural networks assume that inputs and outputs are independent of each other, the output of recurrent neural networks depend on the prior elements within the sequence. While future events would also be helpful in determining the output of a given sequence, unidirectional recurrent neural networks cannot account for these events in their predictions. A simple RNN architecture has a feedback loop computes the values of the hidden units and the output after  time steps. The weights associated with the network are shared temporally. Each recurrent layer has two sets of weights; one for the input and the second one for the hidden unit. The last feedforward layer, which computes the final output for the kth time step is just like an ordinary layer of a traditional feedforward network.


%  Each vertex $v$ stores a local information via feature representation $h_v$, and each edge $e$ stores local information via one-dimensional edge representation $g_e$. The local information for each node $v$ can be shared with their set of neighbouring vertices that results into new feature vector representation $h'_v$. The act of sharing information with vertices is known as message propagation in GNN. There exist multiple ways of message propagation. The final graph structure is represented as a global feature representation $y$ containing graphwide attributes. GNN essentially calculates a set of output feature representations for the vertices $h_v$, edges $g_e$, and complete graph $y$ respectively. For instance, let say a source code snippet is represented as graph, where the functions are vertices in the graph and the edges defines the control flow between functions. Graph-wide feature may represent if the code snippet is malicious.


% learns the node embedding for each node in the graph and aggregate the embedding from all nodes to produce graph embeddings.  

% The final state $x_n$ of the vertex $v_i$ is called final node embedding. 
% GNNs learn embeddings for each node in the graph and aggregate the node embedding to produce graph embeddings. In most general form, the learning process in GNN utilizes the graphical structure and input node embeddings:
% \begin{equation}
%     h_i^{(l)} = f_{\mbox{filter}}(A,H^{(l-1)})
% \end{equation}




% \subsection{GNN Computational Models}
% Fundamentally, a GNN is an algorithm that leverages the graph connectivity to learn and model the relationships between vertices. Through an iterative process that depends on the graph structure, the GNN takes the input edge, vertex, and graph feature vectors (representing their known attributes) and transforms them into output feature vectors (representing the target predictions).
% GNN execution stages are broadly divided into three stages: 
% \begin{itemize}
%     \item \textbf{Pre-processing Model}: This step is performed to prepare the graph structure to a general form that later stages can compute, simplify the graph structure, or to encode additional information that may help in graph-level prediction.
%     \item \textbf{Propagation Model}: GNN represents each node with a $d$-dimensional vector $h_v$ which contains the information of its neighborhood. 
%     $$h_v = f(x_v,x_{co[v]},h_{ne[v]},x_{ne[v]})$$
%      where $x_co[v]$ denotes the features of the edges connecting with $v$, $h_ne[v]$ denotes the embedding of the neighboring nodes of $v$, and $x_ne[v]$ denotes the features of the neighboring nodes of $v$. The function $f$ is the transition function that projects these inputs onto a $d$-dimensional space. Since we are seeking a unique solution for $h_v$, we can apply Banach fixed point theorem and rewrite the above equation as an iteratively update process. Such operation is often referred to as message passing or neighborhood aggregation. The output of the GNN is computed by passing the state $h_v$ as well as the feature $x_v$ to an output function g. 
%     $$o_v=g(h_v,x_v)$$
%     The feature vector of each vertex $v$ is updated using aggregate-combine function iteratively. To update the edges, attributes from the edge itself, the connected vertices, and the graph are aggregated into a single set and combined to yield a new edge feature vector. Similarly, updating the vertices implies aggregating the feature vectors from neighboring vertices  and combining them to obtain a new feature vector. Note that each step or layer updates each edge and vertex with information coming from neighbours located at a single hop. Thus, the iterative process allows to gradually account for relations of increasingly distant nodes and edges. Additionally, in each successive layer, the graph may be coarsened by means of pooling [168] or the neighbourhood set changed by means of layer sampling [65]. 
%     \item \textbf{Readout or Pooling Model}: If the graph has a global feature vector, then it is updated once after the edge and node updates are completed. The final output is either an edge/node embedding, which is a low-dimensional feature vector that represents edge- or node-specific information, or a graph embedding summarizing the information about the entire output graph instead. When we need the representations of high-level subgraphs or graphs, pooling modules are needed to extract information from nodes.
% \end{itemize}

% The aggregation process (equation~\ref{eq:gat-agg}) for node $v$ is a function of node embedding $h_v$ of all neighboring nodes $\N(v)$ from previous iteration $k-1$ iterations, where $\alpha_{uv}$ is the attention value for node $u$ and $v$. The update message $a_v$ (equation~\ref{eq:gat-up}) is used to update node $v$ learned representation using activation function $\sigma$.
% Graph Attention Networks (GATs) and Graph Convolutional Networks (GCNs) are both popular methods for node-level representation learning on graphs. Here are some advantages of GAT over GCN:

% GATs allow for more fine-grained attention: Unlike GCNs, GATs use attention mechanisms to assign different weights to different nodes in the graph when aggregating information from neighbors. This allows GATs to learn more fine-grained representations that capture the relative importance of different nodes for each node in the graph.

% GATs are more expressive: GATs are more expressive than GCNs because they can capture more complex relationships between nodes in the graph. This is because GATs use multi-head attention, which allows them to capture different aspects of the graph structure simultaneously.

% GATs are more flexible: GATs are more flexible than GCNs because they can handle graphs with varying degrees of sparsity and heterogeneity. This is because GATs use attention mechanisms, which can adapt to the sparsity and heterogeneity of the graph.

% GATs are more interpretable: The attention weights learned by GATs can be used to interpret the learned node embeddings. This can be useful for understanding how the model is making predictions and for identifying important nodes in the graph.

% Overall, GATs are a more powerful and flexible approach to node-level representation learning on graphs, but they can also be more computationally expensive than GCNs. The choice between GAT and GCN depends on the specific application and the computational resources available.\


    % \item \textbf{Link-level Classification:} Each edge $e$ is characterized by its feature $X_e$ and associated with a ground-truth class $y_e$. Given a partially labeled graph $\G$, the goal is to predict the relationship between nodes in graphs and predict if two nodes have a connection in between. 

==> commented_subash.tex <==
\usepackage{comment}

\subsection{Evaluation}

    The authors are working on developing metrics to evaluate the performance of privacy preserving GNNS. One such metric, presented by Lie et al. \cite{li2020adversarial}, focuses on prediction accuracy for link and utility attributes from the embeddings. They compared different models based on their ability to correctly categorize edges and non-edges for link prediction, as well as classify utility attributes using multi-layered perceptron and SVM. The APGE model provided the best privacy protection and utility retention using the Yale and Rochester graph datasets, with an average Macro-F1 score of 0.549 on the private attribute.

    Similarly, \cite{wang2021privacy} evaluates the efficacy of their model using two approaches: link prediction without or with node privacy protection and node classification with link privacy protection. 
    The first approach prioritizes link prediction as their primary learning task and node classification as the privacy protection. On the other hand, the second approach prioritized node classification as the primary learning task, and link prediction as the privacy protection task. Results indicated that link prediction without node privacy protection achieved AUCs above 90\% however they were found susceptible to leak node privacy while link prediction with node privacy protection indicated drop in link prediction accuracies however it maintained near perfect node privacy. 

    \subsection{Trade off between Privacy \& Utility}

    And in adversarial privacy-
    preserving \cite{liao2021information, li2020adversarial, wang2021privacy}, how to control the balance between the prediction performance and
    privacy protection is still not well discussed. 


==> deleted_trisha.tex <==


% \noindent\textbf{Problem Statement.} Consider a source code snippet consisting of various functions. To translate the code snippet into graph form: let node $v_i \in \V$ corresponds to a function, and the edges $\E$ correspond to the logical control flow between functions from the source code. The parameters of the function (e.g., variables, syntax, tokens etc) can be represented as node feature vector $X_\V$ and interaction of data between functions (e.g., the flow of values, data types) can be represented as edge features $X_\E$. Each node $v_i\in \V$ is connected to set of nodes denoted by neighborhood $\N(v_i)$. Assume that there are $y$ classes, where $y \in \{y_1, y_2, \dots ,y_c\}$ set of $c$ classes. The classification task on the problem statement can be categorized into two broad levels:


% \begin{itemize}
%     \item \textbf{Node-level Classification:} In node-level classification, a subset of node $\V$ is associated with a ground-truth class $y$. Given a partially labeled graph $\G$, the goal is to leverage these labeled nodes to predict the classes of the remaining unlabeled node. For the problem statement above, example of classification task includes classification of variable and function.
    
%     \item \textbf{Edge-level Classification:} In edge-level classification, a subset of edge $\E$ is associated with a ground-truth class $y$. Given a partially labeled graph $\G$, the goal is to leverage these labeled edges to predict the classes of the remaining unlabeled edge. For the problem statement above, example of classification task includes \trisha{stop here.}
    
    
%     \item \textbf{Graph-level Classification:} In graph-level, the classification task involves predicting the class of whole graph. For our problem statement described above, the classification task involves software vulnerability detection, code quality assessment, software library identification, software language identification.

%     % \shaswata{There is also edge level classification where a relation connecting two nodes is classified. For example anomalous network packet classification.}
% \end{itemize}


==> draft.tex <==
% #####################################

% Anomaly Detection
Anomaly detection is the first phase of run-time prevention, aiming to identify suspicious items, events, network traffic, or observations that exhibit significantly distinctive characteristics from standard patterns or behaviors. A change in operational conditions is crucial for ensuring seamless operations. Such an anomaly can occur in various ways like abnormal login attempts, different user behavior, sudden change in network traffic, inappropriate change in system behavior, etc. For example, in industrial IoT, such detection ensures seamless pipeline operations. In social networks, such can detect spam, malicious activity, and fake data to maintain transparency. In clouds and servers, such can help prevent DoS and numerous other attacks. Using GNN accompanied by GCN, spatial features of such events and traffics are detected, which also helps in computing Graph Anomaly Loss (GAL). Also, there are other GNN derivatives in practice for the task, like Graph Deviation Network (GDN), Relevance-aware Anomalous Users detection (RAU-GNN), Graph Attention Network (GAT), One Class Graph Neural Network (OCGNN), One-Class Temporal Graph Attention Neural Network (OCTGAT), etc.

% Vulnerability Detection
Vulnerability identification is the proactive process of identifying the persisting loopholes in the system to prevent any possible future cyberattack scopes. Such can exist in source code, application patch updates, firewalls, and security policies \& procedures. Early vulnerability identification is crucial to address the weakness in the system, underlying infrastructure, support systems, and applications rather than cleaning post-attack. If such vulnerabilities remain unidentified, attackers can exploit them to execute their malicious intent. To tackle such problems, GNN is used to learn semantics. Utilizing such a feature, numerous GNN models have evolved like Revisiting Graph Neural Network Vulnerability Detection (ReGVD), Degree-free GCN (DR-GCN), etc.

% Intrusion Detection
Intrusion detection refers to passively detecting malicious operations or network traffic in the system and generating alerts when detected. Based on such warnings, the security analyst at SOC can respond with timely measures to remediate the occurring threat. Moreover, the detection provides added benefits, such as enabling the intrusion prevention system (IPS), which aids in protecting the operations. In cybersecurity, intrusion detection can be implemented as either host (HIDS) or network-based (NIDS). In both cases, such detection can occur by detecting malicious signatures, deriving from an anomaly, or utilizing both as a hybrid. GNN's potential to adapt massive topological information helps in detecting such malicious activities. Edge-based Residual Graph Attention Network (E-ResGAT) and GNN-based Deep Belief Network (DBF) are few among the GNN derivatives.

% Malware Detection
Malware is one of the most serious security concerns in cybersecurity, acting autonomously by exploiting the vulnerabilities of a system. This includes viruses, worms, and Trojan horses. Malware detection is the process of monitoring the installed files and applications in the system for potential threats. Such gets achieved in numerous ways, like detecting signatures, heuristic analysis, sandbox analysis, etc. GNN's capability to apprehend the relationship between entities helps for such detection. The learning then gets used in numerous derivation models. For example, GraphSAGE-JK, CGDroid, Deep Graph Convolution neural network (DGCNN), and MatchGNet are a few. 

% What is research & report & type overview of R&R
Contradictory to active run-time prevention, \textit{Research \& Report} refers to passively conducting experiments in a controlled environment and maintaining a threat intelligence to support run-time prevention scopes. Whereas vulnerability identification puts more effort into identifying run-time system loopholes, Research scopes orbit over the security of the employed ML models. Due to the high reliance on the ML models to ensure security, it is crucial to address the protection of such models from adversarial attacks. Therefore, continuous research on adversarial attack possibilities over the GNN models and using such models are essential. On the other hand, all information gathered through run-time prevention and research needs to be collected. All such findings are crucial to be \textit{Reported} to maintain threat intelligence for the models to learn from as cyberattack patterns evolve with time, making adaptation essential.

% Adversarial attacks on & using GNN

% Cyber Threat Intelligence


% #####################################

